Deep probabilistic model for lossless scalable point cloud attribute compression

In recent years, several point cloud geometry compression methods that utilize advanced deep learning techniques have been proposed, but there are limited works on attribute compression, especially lossless compression. In this work, we build an end-to-end multiscale point cloud attribute coding method (MNeT) that progressively projects the attributes onto multiscale latent spaces. The multiscale architecture provides an accurate context for the attribute probability modeling and thus minimizes the coding bitrate with a single network prediction. Besides, our method allows scalable coding that lower quality versions can be easily extracted from the losslessly compressed bitstream. We validate our method on a set of point clouds from MVUB and MPEG and show that our method outperforms recently proposed methods and on par with the latest G-PCC version 14. Besides, our coding time is substantially faster than G-PCC.

==> basic-block-diagram.tex <==

	
	\begin{adjustbox}{width=0.5\textwidth}
%		\tikzstyle{font} = {definition}
		


	\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	%uncomment if require: \path (0,466); %set diagram left start at 0, and has height of 466
	
		%Straight Lines  l1 start
	\draw    (125,180.88) -- (157.63,180.88) ;
	\draw [shift={(160.63,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	%Straight Lines  l1 short
	\draw    (257.86,180.88) -- (303.75,180.88) ;
	\draw [shift={(306.75,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
		
	
	%Straight Lines l1 long
	\draw    (341,180) -- (623.07,181.1) ;
	\draw [shift={(626.07,181.11)}, rotate = 180.22] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	
	
	%Straight Lines  l1 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (730.81,180.88) -- (773,180.88) ;
	\draw [shift={(776,180.88)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	
	
	%Straight Lines  l2 short
	\draw    (318.48,353.94) -- (364.37,353.94) ;
	\draw [shift={(367.37,353.94)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines  l2 long
	\draw    (407,353.94) -- (562.89,354.96) ;
	\draw [shift={(565.89,354.98)}, rotate = 180.38] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;






	%Straight Lines l1 c l2 
	\draw    (279.37,180.88) -- (279.37,330.06) ;
	\draw [shift={(279.37,333.06)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines l3
	\draw    (376.17,527) -- (413.06,527) ;
	\draw [shift={(416.06,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines  l3
	\draw    (433.3,527) -- (508.63,527) ;
	\draw [shift={(511.63,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	%Straight Lines  l2 c l3
	\draw    (337.06,353.94) -- (337.06,503.13) ;
	\draw [shift={(337.06,506.13)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	
	%Straight Lines  up l3 to l2
	\draw    (613.47,527) -- (633.03,527) -- (633.03,377.82) ;
	\draw [shift={(633.03,374.82)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;



	%Straight Lines  up l2 to l1
	\draw    (666.14,353.94) -- (685.7,353.94) -- (685.7,204.75) ;
	\draw [shift={(685.7,201.75)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	%Straight Lines  l2 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (685.7,353.94) -- (767,353.94) ;
	\draw [shift={(770,353.94)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
	%Straight Lines l3 last
	\draw  [dash pattern={on 4.5pt off 4.5pt}]  (633.03,527) -- (773,527) ;
	\draw [shift={(776,527)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;

	
	

		%Shape: Rectangle  encoder1
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (161,160) -- (261,160) -- (261,201.75) -- (161,201.75) -- cycle ;
	%Shape: Rectangle  decoder1
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (627.59,160) -- (727.59,160) -- (727.59,201.75) -- (627.59,201.75) -- cycle ;
		%Rounded Rectq1
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (306.75,168.35) .. controls (306.75,163.74) and (310.48,160) .. (315.1,160) -- (340.19,160) .. controls (344.81,160) and (348.55,163.74) .. (348.55,168.35) -- (348.55,193.4) .. controls (348.55,198.01) and (344.81,201.75) .. (340.19,201.75) -- (315.1,201.75) .. controls (310.48,201.75) and (306.75,198.01) .. (306.75,193.4) -- cycle ;
	% Text Node
	\draw (209,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. I};
	% Text Node
	\draw (327,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (676,180) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. I};
	
	
	
			%Shape: Rectangle  encoder2
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (217.25,333.06) -- (317.25,333.06) -- (317.25,374.82) -- (217.25,374.82) -- cycle ;
		%Shape: Rectangle  %decoder 2
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (565.92,333.06) -- (665.92,333.06) -- (665.92,374.82) -- (565.92,374.82) -- cycle ;
		%Rounded Rect q2
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (367.09,341.61) .. controls (367.09,337) and (370.83,333.26) .. (375.44,333.26) -- (400.54,333.26) .. controls (405.16,333.26) and (408.89,337) .. (408.89,341.61) -- (408.89,366.66) .. controls (408.89,371.28) and (405.16,375.01) .. (400.54,375.01) -- (375.44,375.01) .. controls (370.83,375.01) and (367.09,371.28) .. (367.09,366.66) -- cycle ;
		% Text Node
	\draw (266,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. II};
		% Text Node
	\draw (388,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (615,354) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. II};
	
	
	
	
	
	
	
		%Shape: Rectangle %encoder 3
	\draw  [color={rgb, 255:red, 22; green, 58; blue, 68 }  ,draw opacity=1 ][fill={rgb, 255:red, 219; green, 238; blue, 243 }  ,fill opacity=1 ] (275.94,506.13) -- (375.94,506.13) -- (375.94,547.88) -- (275.94,547.88) -- cycle ;
	%Shape: Rectangle decoder 3
	\draw  [color={rgb, 255:red, 86; green, 40; blue, 4 }  ,draw opacity=1 ][fill={rgb, 255:red, 253; green, 235; blue, 221 }  ,fill opacity=1 ] (512.25,506.13) -- (612.25,506.13) -- (612.25,547.88) -- (512.25,547.88) -- cycle ;
	
		%Rounded Rect q3
	\draw  [color={rgb, 255:red, 51; green, 63; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 235; green, 241; blue, 223 }  ,fill opacity=1 ] (416.08,514.48) .. controls (416.08,509.87) and (419.82,506.13) .. (424.43,506.13) -- (449.53,506.13) .. controls (454.14,506.13) and (457.88,509.87) .. (457.88,514.48) -- (457.88,539.53) .. controls (457.88,544.14) and (454.14,547.88) .. (449.53,547.88) -- (424.43,547.88) .. controls (419.82,547.88) and (416.08,544.14) .. (416.08,539.53) -- cycle ;
	
		% Text Node
	\draw (324,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Enc. III};
		% Text Node
	\draw (436,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Q};
	% Text Node
	\draw (561.5,527) node [anchor=center][inner sep=0.75pt]  [font=\small,xscale=2.25,yscale=2.25] [align=left] {Dec. III};
	










	% Text Node
\draw (750,214) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{1}$};	
% Text Node
\draw (675,387) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{2}$};
% Text Node
\draw (621,560) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$z^{3}$};



	% Text Node
\draw (470,209) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{1}$};	
\draw (470,383) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{2}$};	
% Text Node
\draw (470,556) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$L^{3}$};	




% Text Node
\draw (804,180) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( F\ |\ z^{1})$};

% Text Node
\draw (804,354) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( L^{1} \ |\ z^{2})$};	
	% Text Node
\draw (804,527) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$p( L^{2} \ |\ z^{3})$};


% Text Node
\draw (90,180) node [anchor=west][inner sep=0.75pt]  [font=\small,xscale=2.5,yscale=2.5]  {$F$};
	
	
	
	
\end{tikzpicture}

	
\label{systemooverview}
		
\end{adjustbox}


==> maskAlgo.tex <==
\begin{algorithm2e}[h]
\SetAlgoLined
\SetKwInOut{Input}{Input}
 \small
%\SetKwInOut{Output}{Output}
\KwIn{$mask\_type$} 
%\KwOut{partitioning flags: $fl$, output bitstream: $bits$}
$kernel\_size \leftarrow k_D*k_H*k_W$\\
$mask \leftarrow$ $ ones\_like(kernel)$\\
$mask\left[kernel\_size//2+ mask\_type==B,:,: \right]=0$\\
$kernel=kernel*mask$
       
\caption{Mask construction and application}
\label{algo:maskalg}
\end{algorithm2e}
%\setlength{\textfloatsep}{0pt}
% $kernel\_size=kernel.size()$\\

==> resultTable.tex <==

\begin{table}[t]
\caption{Comparions of our method against G-PCC v14 and VoxelDNN}
\resizebox{0.99\linewidth}{!}{ \begin{tabular}{|P{0.1cm}|l|P{1.2cm}||R{0.7cm}|R{1.4cm}|R{0.7cm}|R{1.4cm}|}
\cline{3-7}
% \multicolumn{2}{|c||}{\begin{bf} Test PC \end{bf}}
\multicolumn{2}{c|}{}
& \begin{bf} G-PCC \end{bf}
& \multicolumn{2}{c|}{\begin{bf}VoxelDNN\end{bf}}
& \multicolumn{2}{c|}{\begin{bf}SparseVoxelDNN\end{bf}}
\\
\cline{2-7}
\multicolumn{1}{c|}{}&Point Cloud & bpov&bpov&Gain over G-PCC &bpov&Gain over G-PCC\\
\hline

\multirow{3}{*}{\rotatebox[origin=c]{90}{MVUB}}&Phil& 1.15 &0.82 &-28\%& 0.40 &-66\%  \\ 
\cline{2-7}
&Ricardo&1.07 &0.75 &-29\%& 0.35&-67\% \\
\cline{2-7}
&\textbf{Average}  &\textbf{1.11}  &\textbf{0.79} &\textbf{-28.5\%} & \textbf{0.37}&\textbf{-66.4\%}  \\
\cline{2-7}
\hline



\multirow{5}{*}{\rotatebox[origin=c]{90}{8i}}&Redandblack &1.09  &0.70 &-36\%& 0.30&-64\% \\
\cline{2-7}
&Loot &0.95&0.61 &-36\% &0.33 & -65\%\\
\cline{2-7}
&Thaidancer&1.00 &0.66 &-34\%&0.32 &-68\% \\
\cline{2-7}
&Boxer&0.95  &0.59 &-38\%& 0.30&-68\% \\
\cline{2-7}
&\textbf{Average} &\textbf{1.00} &\textbf{0.64}& \textbf{-36.0\%}&\textbf{0.34} &\textbf{-66.5\%} \\
\hline



\multirow{4}{*}{\rotatebox[origin=c]{90}{CAT1}}&Frog &1.92   &1.70 &-10\%& 1.23&-36\%  \\
\cline{2-7}
&Arco Valentino &4.85 &4.99 &+3\%& 3.03&-38\% \\
\cline{2-7}
&Shiva&3.67 & 3.50 &-4\%&2.66&-28\% \\
\cline{2-7}
&\textbf{Average} &\textbf{3.48} &\textbf{3.40} &\textbf{-3.8\%}&\textbf{2.31} &\textbf{-33.6\%}\\
\hline



\multirow{3}{*}{\rotatebox[origin=c]{90}{USP}}&BumbaMeuBoi&5.41   &5.07 &-6\%& 2.52&-53\%  \\
\cline{2-7}
&RomanOiLight& 1.86  &1.62 &-13\%& 1.52&-19\% \\
\cline{2-7}
&\textbf{Average}  &\textbf{3.64}  &\textbf{3.35} &\textbf{-9.6\%}&\textbf{2.02}&\textbf{-35.8\%}  \\
\cline{2-7}

\hline
\hline
\end{tabular}}
\label{table:resulttable}
%\noalign{
\vskip 3mm  
\end{table}


==> training_set.tex <==
\begin{table}[t]
\caption{Number of blocks in the training sets of each model}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lR{0.8cm}R{0.8cm}R{0.8cm}R{1.2cm}R{1cm}}
\hline
\begin{bf}  \end{bf}
&\begin{bf}MVUB\end{bf}
& \begin{bf}8i\end{bf} 
&\begin{bf}CAT1\end{bf}
& \begin{bf}Owlii\end{bf} 
& \begin{bf}Total\end{bf} \\
\hline
Block 64 & 317763 &235369 & 2499 & 358834 & 914465\\
\hline
\vspace{0.1mm}
\end{tabular}}
\label{table:noblocks}
\end{table}
